Beurling-type density criteria for system identification

This paper addresses the problem of identifying a linear time-varying (LTV) system characterized by a (possibly infinite) discrete set of delay-Doppler shifts without a lattice (or other geometry-discretizing) constraint on the support set. Concretely, we show that a class of such LTV systems is identifiable whenever the upper uniform Beurling density of the delay-Doppler support sets, measured uniformly over the class, is strictly less than 1/2. The proof of this result reveals an interesting relation between LTV system identification and interpolation in the Bargmann-Fock space. Moreover, we show that this density condition is also necessary for classes of systems invariant under time-frequency shifts and closed under a natural topology on the support sets. We furthermore show that identifiability guarantees robust recovery of the delay-Doppler support set, as well as the weights of the individual delay-Doppler shifts, both in the sense of asymptotically vanishing reconstruction error for vanishing measurement error.

==> def.tex <==
% !TEX root = SystemIdentificationJournal.tex

% To define macros
\makeatletter
\def\iffirsttoken#1#2{
	\expandafter\def\expandafter\@first@token\expandafter{\@car#1\@nil}
	\expandafter\ifx\@first@token#2\relax
	\expandafter\@firstoftwo
 \else
  	\expandafter\@secondoftwo
 \fi
}


% Theorems
\newtheorem{thm}{Theorem}
\newtheorem{cor}[thm]{Corollary}   % Turned off theorem numbering
\newtheorem{prop}{Proposition}
\newtheorem{defn}{Definition}
\newtheorem{ex}{Example}
\newtheorem{lem}[thm]{Lemma}

% Mathematical functions
\DeclareMathOperator{\sgn}{sgn}
\newcommand{\closure}[1]{\overline{#1}}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\real}{Re}
\DeclareMathOperator{\imag}{Im}
\renewcommand{\Re}[1]{\real\left\{#1\right\}}
\renewcommand{\Im}[1]{\imag\left\{#1\right\}}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\cont}{cont}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\indic}{I}
\newcommand{\abs}[1]{\left|#1\right|}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\erf}{erf}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\dist}{dist}

% Triangleq
\renewcommand{\triangleq}{\vcentcolon=}
\newcommand{\reversetriangleq}{=\vcentcolon}

% Minimization problems
\DeclareMathOperator*{\minimize}{minimize\ }
\DeclareMathOperator*{\maximize}{maximize\ }
\DeclareMathOperator{\st}{\ subject\ to\ }

% Sets
\newcommand{\C}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\torus}{\mathbb{T}}

% Inequalities
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}

% Spaces
\newcommand{\schwartzSpace}[1]{\mathcal{S}(#1)}
\newcommand{\measSpace}[1]{\mathcal{M}(#1)}
\newcommand{\measSpacep}[2]{\mathcal{M}^{#1}(#2)}
\newcommand{\borelAlgebra}[1]{\mathcal{B}(#1)}
\newcommand{\dmeas}[2]{\mathrm{d}#1\left( #2 \right)}
\newcommand{\linfty}[1]{\ell^\infty(#1)}

% Norms and inner products
\newcommand{\innerProd}[2]{\left\langle #1, #2 \right\rangle}
\DeclareMathOperator*{\tv}{TV}
\newcommand{\normTV}[1]{\left\|#1\right\|_{\tv}}
\newcommand{\normOp}[1]{\left\|#1\right\|}
\newcommand{\normInfty}[1]{\left\|#1\right\|_{\infty}}
\newcommand{\normltwo}[1]{\left\|#1\right\|_{\ell_2}}
\newcommand{\normLtwo}[1]{\left\|#1\right\|_{L^2}}
\newcommand{\normLone}[1]{\left\|#1\right\|_{L^1}}
\newcommand{\normLinfty}[1]{\left\|#1\right\|_{L^\infty}}
\newcommand{\normlinfty}[1]{\left\|#1\right\|_{\ell^\infty}}

